Object-oriented lexical encoding of multiword expressions: Short and sweet

Multiword expressions (MWEs) exhibit both regular and idiosyncratic properties. Their idiosyncrasy requires lexical encoding in parallel with their component words. Their (at times intricate) regularity, on the other hand, calls for means of flexible factorization to avoid redundant descriptions of shared properties. However, so far, non-redundant general-purpose lexical encoding of MWEs has not received a satisfactory solution. We offer a proof of concept that this challenge might be effectively addressed within eXtensible MetaGrammar (XMG), an object-oriented metagrammar framework. We first make an existing metagrammatical resource, the FrenchTAG grammar, MWE-aware. We then evaluate the factorization gain during incremental implementation with XMG on a dataset extracted from an MWE-annotated reference corpus.

==> Images/Images/tags-fig.tex <==
% \begin{figure}[htbp]
   \centering {\small

   \begin{tikzpicture}[node distance=.2cm,level distance=.6cm]
     \node(s){S}
     child{node (np){NP$\downarrow$}}
     child[sibling distance=.6cm]{node (vp){VP}
       child{node{V}
         child{node{happen}}}};
     \node[below left=.2cm and .1cm of np](npr){NP}
     child{node(zen){N}
       child{node{rains}}};
     \node[below left=.2cm and 2.6cm of vp](vpr){N}
     child{node{N}
       child{node{acid}}}
     child[sibling distance=.3cm]{node(vpf){N$\star$}};
     \path[->,dotted,color=black!70,thick]
     (npr) edge (np);
     \path[->,dashed,color=black!70,thick]
     (vpr) edge [bend left=30] (zen)
     (vpf) edge [bend right=30] (zen);
     %\node[below right=2.4cm and .5cm of s]{S}
     \node[below right=0.cm and 2.4cm of s]{S}
     child{node{NP}
       child{node(zenp){N}
         child{node{N}
           child{node{acid}}}
         child[sibling distance=.6cm]{node{N}
           child{node{rains}}}}
     }
     child[sibling distance=.8cm]{node{VP}
       child{node{V}
         child{node{happen}}}};
     \node[left=.4cm of zenp]{\Large $\Rightarrow$};
   \end{tikzpicture}
%   \vspace{-.5cm}
 }
%   \caption{Tree rewriting in TAG.}
%   \label{fig1}
% \end{figure}


